Boundary Arm Exponents for SLE$(\kappa)$

We derive boundary arm exponents for SLE. Combining with the convergence of critical lattice models to SLE, these exponents would give the alternating half-plane arm exponents for the corresponding lattice models.

==> introduction.tex <==
Schramm-Loewner evolution (SLE) was introduced by Oded Schramm \cite{SchrammFirstSLE} as the candidates for the scaling limits of interfaces in 2D critical lattice models. It is a one-parameter family of random fractal curves in simply connected domains from one boundary point to another boundary point, which is indexed by a positive real $\kappa$.
Since its introduction, it has been proved to be the limits of several lattice models:
$\SLE_2$ is the limit of Loop Erased Random Walk and $\SLE_8$ is the limit of the Peano curve of Uniform Spanning Tree \cite{LawlerSchrammWernerLERWUST}, $\SLE_3$ is the limit of the interface in critical Ising model and $\SLE_{16/3}$ is the limit of the interface in FK-Ising model \cite{CDCHKSConvergenceIsingSLE}, $\SLE_4$ is the limit of the level line of discrete Gaussian Free Field \cite{SchrammSheffieldDiscreteGFF} and $\SLE_6$ is the limit of the interface in critical Percolation \cite{SmirnovPercolationConformalInvariance}.

In the study of lattice models, arm exponents play an important role. Take percolation for instance, Kesten has shown that \cite{KestenScalingRelationPercolation} in order to understand the behavior of percolation near its critical point, it is sufficient to study what happens at the critical point, and many results would follow from the existence and values of the arm exponents. To be more precise, consider critical percolation with fixed mesh equal to 1, and for $n\ge 2$, consider the the event $E_n(z, r, R)$ that there exist $n$ disjoint crossings of the annulus $A_z(r, R):=\{w\in\C: r<|w-z|<R\}$, not all of the same color. People would like to understand the decaying of the probability of $E_n(z, r,R)$ as $R\to\infty$. It turns out that this probability decays like a power in $R$, and the exponent is called plane arm exponents.
There are another related quantities, called half-plane arm exponents. In this case, consider critical percolation in the upper-half plane $\HH$, and for $n\ge 1, x\in\R$, define $H_n(x, r, R)$ to be the event that there exist $n$ disjoint crossings of the semi-annulus $A_x^+(r, R):=\{w\in\HH: r<|w-x|<R\}$.
After the identification between $\SLE_6$ and the limit of critical percolation on triangular lattice \cite{SmirnovPercolationConformalInvariance}, one could derive these exponents via the corresponding arm exponents for $\SLE_6$ \cite{SmirnovWernerCriticalExponents}:
\[\PP\left[E_n(z, r,R)\right]= R^{-\alpha_n+o(1)},\quad \PP\left[H_n(x, r,R)\right]=R^{-\alpha_n^++o(1)},\quad \text{as }R\to\infty,\]
where
\[\alpha_n:=(n^2-1)/12,\quad \alpha_n^+:=n(n+1)/6.\]

In this paper, we derive boundary arm exponents for $\SLE_{\kappa}$. Combining with the identification between the limit of critical lattice model and $\SLE$ curves, these exponents for $\SLE$ would imply the arm exponents for the corresponding lattice models.

Fix $\kappa>4$ and let $\eta$ be an $\SLE_{\kappa}$ in $\HH$ from 0 to $\infty$. Suppose that $y\le 0<\eps\le x$ and let $T$ be the first time that $\eta$ swallows the point $x$ which is almost surely finite when $\kappa>4$. We first define the crossing event $H_{2n-1}$ (resp. $\hat{H}_{2n}$) that $\eta$ crosses between the ball $B(x,\eps)$ and the half-infinite line $(-\infty, y)$ at least $2n-1$ times (resp. at least $2n$ times) for $n\ge 1$. To be precise with the definition, we need to introduce a sequence of stopping times.
Set $\tau_0=\sigma_0=0$. Let $\tau_1$ be the first time that $\eta$ hits the ball $B(x,\eps)$ and let $\sigma_1$ be the first time after $\tau_1$ that $\eta$ hits $(-\infty, y)$. For $n\ge 1$, let $\tau_n$ be the first time after $\sigma_{n-1}$ that $\eta$ hits the connected component of $\partial B(x,\eps)\setminus \eta[0,\sigma_{n-1}]$ containing $x+\eps$ and let $\sigma_n$ be the first time after $\tau_n$ that $\eta$ hits $(-\infty, y)$. Define $H_{2n-1}(\eps, x, y)$ to be the event that $\{\tau_n<T\}$.
Define $\hat{H}_{2n}(\eps, x, y)$ to be the event that $\{\sigma_n<T\}$.
In the definition of $H_{2n-1}(\eps, x, y)$ and $\hat{H}_{2n}(\eps, x, y)$,  we are particular interested in the case when $x$ is large. Roughly speaking, the event $H_{2n-1}(\eps, x, y)$ means that $\eta$ makes at least $(2n-1)$ crossings between $B(x,\eps)$ and $(-\infty, y)$. Imagine that $\eta$ is the interface in the discrete model, then $H_{2n-1}(\eps,x,y)$ interprets the event that there are $2n-1$ arms going from $B(x,\eps)$ to far away place. The event $\hat{H}_{2n}(\eps, x, y)$ means that $\eta$ makes at least $2n$ crossings between $B(x,\eps)$ and $(-\infty, y)$. Imagine that $\eta$ is the interface in the discrete model, then $\hat{H}_{2n}(\eps,x,y)$ interprets the event that there are $2n$ arms going from $B(x,\eps)$ to far away place. See Figure \ref{fig::boundaryarms}(a).


\begin{figure}[ht!]
\begin{subfigure}[b]{0.49\textwidth}
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/boundaryarms1}
\end{center}
\caption{This figure indicates $\hat{H}_4$. The stopping times\\ $\tau_1<\sigma_1<\tau_2<\sigma_2<T_x$ are indicated in the figure. }
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\begin{center}\includegraphics[width=0.9\textwidth]{figures/boundaryarms2}
\end{center}
\caption{This figure indicates $H_4$. The stopping times\\ $\sigma_1<\tau_1<\sigma_2<\tau_2<T_x$ are indicated in the figure. }
\end{subfigure}
\caption{\label{fig::boundaryarms} The explanation of the definition of the crossing events. The gray part is the ball $B(x,\eps)$.}
\end{figure}


Next, we define the crossing event $H_{2n}$ (resp. $\hat{H}_{2n+1}$) that $\eta$ crosses between the half-infinite line $(-\infty, y)$ and the ball $B(x,\eps)$ at least $2n$ times (resp. at least $2n+1$ times) for $n\ge 0$. Set $\tau_0=\sigma_0=0$. Let $\sigma_1$ be the first time that $\eta$ hits $(-\infty, y)$ and $\tau_1$ be the first time after $\sigma_1$ that $\eta$ hits the connected component of $\partial B(x,\eps)\setminus \eta[0,\sigma_1]$ containing $x+\eps$. For $n\ge 1$, let $\sigma_n$ be the first time after $\tau_{n-1}$ that $\eta$  hits $(-\infty, y)$ and $\tau_n$ be the first time after $\sigma_n$ that $\eta$ hits the connected component of $\partial B(x,\eps)\setminus \eta[0,\sigma_n]$ containing $x+\eps$.
Define $H_{2n}(\eps, x, y)$ to be the event that $\{\tau_{n}<T\}$.
Define $\hat{H}_{2n+1}(\eps, x, y)$ to be the event that $\{\sigma_{n+1}<T\}$.
In the definition of $H_{2n}(\eps, x, y)$ and $\hat{H}_{2n+1}(\eps, x, y)$. we are interested in the case when $x$ is of the same size as $\eps$ and $y$ is large. Roughly speaking, the event $H_{2n}(\eps, x,y)$ means that $\eta$ makes at least $2n$ crossings between $(-\infty, y)$ and $B(x,\eps)$. Imagine that $\eta$ is the interface in the discrete model, then $H_{2n}(\eps, x, y)$ interprets the event that there are $2n$ arms going from $B(x,\eps)$ to far away place.
The event $\hat{H}_{2n+1}(\eps, x,y)$ means that $\eta$ makes at least $2n+1$ crossings between $(-\infty, y)$ and $B(x,\eps)$. Imagine that $\eta$ is the interface in the discrete model, then $\hat{H}_{2n+1}(\eps, x, y)$ interprets the event that there are $2n+1$ arms going from $B(x,\eps)$ to far away place.
See Figure \ref{fig::boundaryarms}(b).

Note that in the definition of $H_{2n-1}$ and $\hat{H}_{2n}$, we start from $\tau_1$ and
\[H_{2n-1}(\eps, x, y)=\{\tau_1<\sigma_1<\tau_2<\cdots<\tau_n<T\},\quad
\hat{H}_{2n}(\eps, x, y)=\{\tau_1<\sigma_1<\tau_2<\cdots<\tau_n<\sigma_n<T\}.\]
In the definition of $H_{2n}$ and $\hat{H}_{2n+1}$, we start from $\sigma_1$ and
\[H_{2n}(\eps, x, y)=\{\sigma_1<\tau_1<\sigma_2<\cdots<\tau_n<T\},\quad \hat{H}_{2n+1}(\eps, x, y)=\{\sigma_1<\tau_1<\sigma_2<\cdots<\tau_n<\sigma_{n+1}<T\}.\] The two sequences of stopping times are defined in different ways. Readers may wander why we do not define the events using the same sequence of stopping times. We realize that the definition using the same sequence of stopping times causes ambiguity. Therefore, we decide to define these events in the above way. The advantages of the current definition will become clear in the proofs.

We define the arm exponents as follows. Set $\alpha_0^+=0$. For $n\ge 1$ and $\kappa\in (0,8)$, define
\begin{equation}\label{eqn::boundary_arm_formula_less8}
\alpha_{2n-1}^+=n(4n+4-\kappa)/\kappa,\quad \alpha^+_{2n}=n(4n+8-\kappa)/\kappa.
\end{equation}
For $n\ge 1$ and $\kappa\ge 8$, define
\begin{equation}\label{eqn::boundary_arm_formula_greater8}
\alpha_{2n-1}^+=(n-1)(4n+\kappa-8)/\kappa,\quad \alpha_{2n}^+=n(4n+\kappa-8)/\kappa.
\end{equation}

\begin{theorem}\label{thm::boundary_arm_greater4}
Fix $\kappa>4$. The crossing events $H_{2n-1}(\eps, x, y)$ and $H_{2n}(\eps, x, y)$ are defined as above.
Then, for any $y\le 0<\eps\le x$ and $n\ge 1$, we have
\begin{equation}\label{eqn::boundary_arm_greater4_odd}
\PP[H_{2n-1}(\eps, x, y)]\asymp \left(\frac{x}{x-y}\right)^{\alpha_{2n-2}^+}\left(\frac{\eps}{x}\right)^{\alpha_{2n-1}^+},
\begin{comment}
\quad \text{provided }x\ge 8^{2n-1}\eps,
\end{comment}
\end{equation}
\begin{equation}\label{eqn::boundary_arm_greater4_even}
\PP[H_{2n}(\eps, x, y)]\asymp \left(\frac{x}{x-y}\right)^{\alpha_{2n}^+}\left(\frac{\eps}{x}\right)^{\alpha_{2n-1}^+},
\begin{comment}
\quad \text{provided }x-y\ge 8^{2n}\eps,
\end{comment}
\end{equation}
where the constants in $\asymp$ depend only on $\kappa$ and $n$. In particular, fix some $\delta>0$, we have
\[\PP[H_{2n-1}(\eps, x, y)]\asymp \eps^{\alpha_{2n-1}^+},\quad\text{provided }\delta\le x\le 1/\delta, -1/\delta\le y\le 0,\]
\[\PP[H_{2n}(\eps, x, y)]\asymp\eps^{\alpha_{2n}^+},\quad \text{provided }\eps\le x\le \eps/\delta, -1/\delta\le y\le -\delta,\]
where the constants in $\asymp$ depend only on $\kappa, n$ and $\delta$.
\end{theorem}

By a similar proof, we could obtain a similar result as Theorem \ref{thm::boundary_arm_greater4} for $\SLE_{\kappa}(\rho)$ curve in the case that $x$ coincides with the force point. The exponents and a complete proof can be found in \cite[Section 3]{WuPolychromaticArmFKIsing}, where the conditions are loosen such that the force point may not be equal to $x$. One may also study the arm exponents for $\kappa\in(0,4]$. Whereas, when $\kappa\le 4$, the $\SLE$ curve does not touch the boundary, thus the above definition of the crossing events is not proper for $\kappa\le 4$. In Section \ref{sec::boundary_less4}, we have Theorem \ref{thm::boundary_arm_alternative} for the crossing events between a small circle and a half-infinite strip, where the arm exponents are defined in the same way as in (\ref{eqn::boundary_arm_formula_less8}). The proof of Theorem \ref{thm::boundary_arm_alternative} also works for $\SLE_{\kappa}(\rho)$ when $x$ coincides with the force point.

\begin{theorem}\label{thm::boundary_arm_hat}
Fix $\kappa\in (4,8)$. Set $\hat{\alpha}_0^+=0$. The crossing events $\hat{H}_{2n}(\eps, x, y)$ and $\hat{H}_{2n+1}(\eps, x, y)$ are defined as above.
For $n\ge 1$, define
\begin{equation}\label{eqn::boundary_arm_formula_hat}
\hat{\alpha}_{2n-1}^+=n(4n+\kappa-8)/\kappa,\quad \hat{\alpha}_{2n}^+=n(4n+\kappa-4)/\kappa.
\end{equation}
Then, for $y\le 0<\eps\le x$ and $n\ge 1$, we have
\begin{equation}\label{eqn::boundary_arm_hat_odd}
\PP\left[\hat{H}_{2n-1}(\eps, x, y)\right]\asymp \left(\frac{x}{x-y}\right)^{\hat{\alpha}_{2n-1}^+}\left(\frac{\eps}{x}\right)^{\hat{\alpha}_{2n-2}^+}, 
\begin{comment}
\quad \text{provided }x-y\ge 8^{2n-1}\eps,
\end{comment}
\end{equation}
\begin{equation}\label{eqn::boundary_arm_hat_even}
\PP\left[\hat{H}_{2n}(\eps, x, y)\right]\asymp \left(\frac{x}{x-y}\right)^{\hat{\alpha}_{2n-1}^+}\left(\frac{\eps}{x}\right)^{\hat{\alpha}_{2n}^+},
\begin{comment}\quad \text{provided }x\ge 8^{2n}\eps,
\end{comment}
\end{equation}
where the constants in $\asymp$ depend only on $\kappa$ and $n$. In particular, fix some $\delta>0$, we have
\[\PP\left[\hat{H}_{2n-1}(\eps, x, y)\right]\asymp\eps^{\hat{\alpha}_{2n-1}^+},\quad \text{provided } \eps\le x\le \eps/\delta, -1/\delta\le y\le -\delta,\]
\[\PP\left[\hat{H}_{2n}(\eps, x, y)\right]\asymp\eps^{\hat{\alpha}_{2n}^+},\quad \text{provided }\delta\le x\le 1/\delta, -1/\delta\le y\le 0,\]
where the constants in $\asymp$ depend only on $\kappa, n$ and $\delta$.
\end{theorem}

It is worthwhile to spend some more words on the relation between $\alpha_n^+$ and $\hat{\alpha}_n^+$. In fact, we can also define the crossing events $\hat{H}_n(\eps, x, y)$ for $\kappa\in [0,4]$ and $\kappa\ge 8$. When $\kappa\le 4$, the $\SLE$ curve does not touch the boundary, thus the exponent $\hat{\alpha}_n^+$ coincides with $\alpha_{n-1}^+$. When $\kappa\ge 8$, the $\SLE$ curve is space-filling, thus the exponent $\hat{\alpha}_{n}^+$ coincides with $\alpha_{n+1}^+$. Whereas, when $\kappa\in (4,8)$, the exponent $\hat{\alpha}_n^+$ is distinct from $\alpha_n^+$ in general. In terms of discrete model, both $\alpha_n^+$ and $\hat{\alpha}_n^+$ interpret the boundary $n$-arm exponents, but their boundary conditions are different.

It is explained in \cite{SmirnovWernerCriticalExponents} that combining the following three facts would imply the arm exponents for the discrete model: (1) Identification between $\SLE_{\kappa}$ and the limit of the interface in critical lattice model; (2) The arm exponents of $\SLE_{\kappa}$;
(3) Crossing probabilities enjoy (approximate) multiplicativity property.  For critical Ising and FK-Ising model on $\Z^2$ with Dobrushin boundary conditions, the convergence to $\SLE_3$ and $\SLE_{16/3}$ respectively is derived in \cite{ChelkakSmirnovIsing, CDCHKSConvergenceIsingSLE}, and the multiplicativity is derived in \cite{ChelkakDuminilHonglerCrossingprobaFKIsing}. Therefore, we could derive the arm exponents for these two models. See more details in \cite{WuPolychromaticArmFKIsing, WuAlternatingArmIsing}. Moreover, the formula of $\alpha^+_{2n-1}$ in (\ref{eqn::boundary_arm_formula_less8}) was predicted by KPZ in \cite[Equations (11.42), (11.44)]{DuplantierFractalGeometry}.

\begin{comment}
For critical Ising model on $\Z^2$ with Dobrushin boundary conditions, we have the alternating half-plane arm exponents: {\color{red}(see Figure for the boundary conditions)}
\begin{equation}
\alpha_{2n-1}^+=n(4n+1)/3,\quad \alpha_{2n}^+=n(4n+5)/3.
\end{equation}

For critical FK-Ising model on $\Z^2$ with Dobrushin boundary conditions, we have the alternating half-plane arm exponents: {\color{red}(see Figure for the boundary conditions)}
\begin{equation}
\alpha_{2n-1}^+=n(3n-1)/4,\quad \alpha_{2n}^+=n(3n+2)/4;\quad \hat{\alpha}_{2n-1}^+=n(3n-2)/4,\quad \hat{\alpha}_{2n}^+=n(3n+1)/4.
\end{equation}
\end{comment}
\smallbreak
\noindent\textbf{Relation to previous results.} The formula of $\alpha_n^+$ and $\alpha_n$ for $\kappa=6$ was obtained in \cite{LawlerSchrammWernerExponent1, SmirnovWernerCriticalExponents}. The exponent $\alpha_1^+$ is related to the Hausdorff dimension of the intersection of $\SLE_{\kappa}$ with the real line which is $1-\alpha_1^+$ when $\kappa>4$. This dimension was obtained in \cite{AlbertsSheffieldDimension}. The most important ingredients in proving Theorem \ref{thm::boundary_arm_greater4} is the Laplace transform of the derivatives of the conformal map in $\SLE$ evolution, which was obtained in \cite{LawlerMinkowskiSLERealLine}.
\smallbreak
\noindent\textbf{Acknowledgment.} The authors acknowledge Hugo Duminil-Copin, Christophe Garban, Gregory Lawler,
Stanislav Smirnov, Vincent Tassion, Brent Werness, and David Wilson for helpful discussions. Hao Wu's work is supported by the NCCR/SwissMAP, the ERC AG COMPASP, the Swiss NSF.
Dapeng Zhan's work is partially supported by NSF DMS-1056840.


